An Efficient and Explanatory Image and Text Clustering System with Multimodal Autoencoder Architecture

We demonstrate the efficiencies and explanatory abilities of extensions to the common tools of Autoencoders and LLM interpreters, in the novel context of comparing different cultural approaches to the same international news event. We develop a new Convolutional-Recurrent Variational Autoencoder (CRVAE) model that extends the modalities of previous CVAE models, by using fully-connected latent layers to embed in parallel the CNN encodings of video frames, together with the LSTM encodings of their related text derived from audio. We incorporate the model within a larger system that includes frame-caption alignment, latent space vector clustering, and a novel LLM-based cluster interpreter. We measure, tune, and apply this system to the task of summarizing a video into three to five thematic clusters, with each theme described by ten LLM-produced phrases. We apply this system to two news topics, COVID-19 and the Winter Olympics, and five other topics are in progress.

==> sections/future_work.tex <==
% NOT USED; INCORPORATED INTO DISCUSSION SECTION
\section{Future Work}

We have fully implemented our system, with two videos each (Chinese and English) on two very different topics, COVID-19 and Winter Olympics.
As discussed in Section~\ref{sec:dataset},
we are applying our pipeline to five additional topics; see Table~\ref{tab:five_topics} for details.
Additionally, we 
will be extending some topics to include additional videos.

\begin{comment}
The first additional topic is topic China's “visa-free” visitor policy, which we expect to show more sympathetic presentations by Chinese sources.
The second concerns the Copa America 2024 Soccer Tournament, where we expect more technical details from English sources.
The third concerns the Beryl Hurricane, expecting discussions of climate change from English sources.
The fourth is self-driving taxis, a very new concern in Chinese news media.
The last is the contaminated cooking oil crisis in China, where we anticipate English commentary to be simply fact-based.
\end{comment}
